A Multifaceted Look at Starlink Performance

In recent years, Low-Earth Orbit (LEO) mega-constellations have emerged as a promising network technology and have ushered in a new era for democratizing Internet access. The Starlink network from SpaceX stands out as the only consumer-facing LEO network with over 2M+ customers and more than 4000 operational satellites. In this paper, we conduct the first-of-its-kind extensive multi-faceted analysis of Starlink network performance leveraging several measurement sources. First, based on 19.2M crowdsourced M-Lab speed test measurements from 34 countries since 2021, we analyze Starlink global performance relative to terrestrial cellular networks. Second, we examine Starlink's ability to support real-time web-based latency and bandwidth-critical applications by analyzing the performance of (i) Zoom video conferencing, and (ii) Luna cloud gaming, comparing it to 5G and terrestrial fiber. Third, we orchestrate targeted measurements from Starlink-enabled RIPE Atlas probes to shed light on the last-mile Starlink access and other factors affecting its performance globally. Finally, we conduct controlled experiments from Starlink dishes in two countries and analyze the impact of globally synchronized "15-second reconfiguration intervals" of the links that cause substantial latency and throughput variations. Our unique analysis provides revealing insights on global Starlink functionality and paints the most comprehensive picture of the LEO network's operation to date.

==> sections/app-ethics.tex <==
\section{Ethics}

To the best of our knowledge, \emph{our work does not raise any ethical concerns}. The M-Lab dataset is publicly accessible and the platform meticulously removes any identifying information of the connections~\cite{mlab-pub}. We do not attempt to pinpoint specific users in this work but only conclude on the aggregated dataset. 
% A majority part of our work is based on rigorous active measurements. Throughout our experiments we took care to mitigate any potential harm to the destination servers. The frequency of our \texttt{ping}, \texttt{tracerute} and \texttt{iRTT} measurements towards cloud data centers was set to once every 2 minutes. Our parallel measurements across two Starlink terminals lasted only \textcolor{red}{N minutes}. We have conducted these measurements with the utmost consideration for maintaining the proper operation of the target systems.

% By adhering to these scientific principles and considering the context of our analysis, we believe that our approach strikes a delicate balance between conducting comprehensive measurements and safeguarding the stability and integrity of the systems under scrutiny.


==> sections/app-mno.tex <==
\section{Top-3 MNOs per Country}\label{app:sec:mno}

%\begin{figure}[htbp]
%	\begin{subfigure}[htbp]{0.4\textwidth}
%		\includegraphics[width=\textwidth]{figures/mlab/temp_mno_operators.png}
%		\caption{\label{fig:temp_mno_operators} \textcolor{red}{Temporary data dump} Top Mobile Network Operators for countries we have data in Mlab}
%	\end{subfigure}
%	\caption{temporary dump}
%\end{figure}

%\textcolor{red}{Make table more presentable}.

%\begin{table}[]
%\centering
%\begin{adjustbox}{width=\columnwidth}
%\begin{tabular}{@{}cccccc@{}}
%\toprule
%\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Inclination\\ angle\end{tabular}}} &
%  \multirow{2}{*}{\textbf{\# Planes}} &
%  \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Altitude\\ {[}km{]}\end{tabular}}} &
%  \multicolumn{3}{c}{\textbf{\# Satellites}} \\
%    \cmidrule(l){4-6}
%      &    &     & \textbf{\begin{tabular}[c]{@{}c@{}}In\\ Position\end{tabular}} & \textbf{Launched} & \textbf{Filed \textcolor{red}{[cite]}} \\
%  \midrule
%53°   & 72 & 550 & 1427                                                           & 1665              & 1584           \\
%53.2° & 72 & 540 & 1508                                                           & 1637              & 1584           \\
%70°   & 36 & 570 & 88                                                             & 305               & 720            \\
%97.6° & 10 & 560 & 184                                                            & 230               & 508           \\
%\bottomrule
%\end{tabular}
%\end{adjustbox}
%    \caption{\label{tbl:starlink_orbits}Starlink orbital shell design and number of operational satellites as of early May 2023. The 53° inclination shell consists of v1.0 satellites and the rest are v1.5 satellites \textcolor{red}{[cite]}} 
%\end{table}

\Cref{tab:top3_mno} lists the top-3 Mobile Network Operators (MNOs) of the countries that are part of our M-Lab dataset.
%
The selection is based on a combination of each AS's rank and the number of M-Lab measurements originating from that AS.


==> sections/discussion.tex <==
\section{Discussion} \label{sec:discussion}

% \headline{Limitations of client-triggered M-Lab measurements.}
% % -> Moved to methodology
% %
% We recognize and acknowledge that the data collected using the NDT tool may be subject to several limitations, which we believe are important to address.
% One such limitation is the potential presence of sampling bias in our dataset.
% Internet speed tests are typically conducted by users who are already experiencing some level of degradation in their Internet service.
% This can introduce a bias towards slower speeds and may not fully represent the true performance of the Internet connection during normal usage.
% %
% Furthermore, the accuracy of geolocation data, which we rely on for more precise analysis, is not flawless.
% While MaxMind self-reports accuracy of over 68\% at a resolution of 25 km [37], multiple studies showed inconsistencies while geolocating IP addresses~\cite{livadariu2020accuracy,scheitle2017hloc,shavitt2011geolocation}.
% %
% Further, M-Lab's Starlink data set only contains one city per country; the USA and Australia are notable exceptions.
% We believe the low precision to be a consequence of Starlink's PoP architecture:
% The PoP IP addresses are likely not mapped to accurate client geolocations.
% We therefore consider the reported geolocations to cover a larger area around the cities.
% %
% Given these limitations, we approached our analysis with caution, particularly when examining fine-grained region-specific information.
% We refrained from drawing definitive conclusions or making generalizations based solely on this level of detail, as it could be influenced by potential biases stemming from inaccurately labeled data.
% Instead, we focused on broader trends and patterns that emerged from the aggregated data at country-level breakup, aiming to provide a comprehensive overview of the network performance while remaining mindful of these inherent limitations.


==> sections/mobility.tex <==
\section{Mobility Analysis}

\textcolor{red}{Responsible: Hendrik}

\textbf{Timeline:}
\begin{enumerate}
    \item May 5: description of the measurements
    \item May 12: initial results
\end{enumerate}

Overall structure:

\begin{enumerate}
\item Pointers here.
\end{enumerate}

Starlink and cellular technology share multiple characteristics: Both networks aim to cover a large outdoor area and provide high-speed and low-latency Internet access.
Cellular networks are already used to provide Internet access to users while they are moving in cars and trains.
The performance of the network connection depends on the deployed cellular infrastructure that must be scaled to handle the peak loads of a crowded train to maintain a high level of service.
Given the similarities of cellular networks and Starlink, we set out to investigate the performance of Starlink in-motion.

To test the network performance in-motion, we rented a convertible car to provide a Starlink dish with a clear view to the sky.
\autoref{fig:mobility_setup_diagram} provides a schematic depiction of our measurement setup.
The Starlink dish was plugged into the Starlink Volcano Mount that was screwed onto a wooden pallet and secured to the backseats of the car with a strap.
Power was delivered to the dish by… Well, let’s see (TODO)!

We established cellular connections to the networks of two mobile network operators (MNOs).
The connections were maintained by two smartphones (model Samsung A23 5G) that were rooted to access detailed information about the cellular link.
We used the application “Network Signal Guru” to log… TODO

A notebook served as our central hub that generated traffic and logged information about the three available network links.
The smartphones were connected over USB while the Starlink dish was accessed over Ethernet through its Power over Ethernet (PoE) power supply.


\begin{figure}[htbp]
  \centering
  \includegraphics[width=\columnwidth]{figures/mobility_setup_diagram.drawio.pdf}
  \caption{\label{fig:mobility_setup_diagram} Our mobile test setup.}
\end{figure}

